Comparative Document Summarisation via Classification

This paper considers extractive summarisation in a comparative setting: given two or more document groups (e.g., separated by publication time), the goal is to select a small number of documents that are representative of each group, and also maximally distinguishable from other groups. We formulate a set of new objective functions for this problem that connect recent literature on document summarisation, interpretable machine learning, and data subset selection. In particular, by casting the problem as a binary classification amongst different groups, we derive objectives based on the notion of maximum mean discrepancy, as well as a simple yet effective gradient-based optimisation strategy. Our new formulation allows scalable evaluations of comparative summarisation as a classification task, both automatically and via crowd-sourcing. To this end, we evaluate comparative summarisation methods on a newly curated collection of controversial news topics over 13 months. We observe that gradient-based optimisation outperforms discrete and baseline approaches in 14 out of 24 different automatic evaluation settings. In crowd-sourced evaluations, summaries from gradient optimisation elicit 7% more accurate classification from human workers than discrete optimisation. Our result contrasts with recent literature on submodular data subset selection that favours discrete optimisation. We posit that our formulation of comparative summarisation will prove useful in a diverse range of use cases such as comparing content sources, authors, related topics, or distinct view points.

==> sections/model_old.tex <==
\section{Method}
We formulate the problem of summarization as prototype learning problem. Given a set of objects $X = \{x_1, x_2, \ldots , x_n \} $, $X \in \mathbb{R}^{n \times d}$ be the given dataset. Goal is to learn a set of prototypes $A \in \mathbb{R}^{m \times d}, \ m << n$ such that $A$ is a good representative of $X$. A prototype is a sample from dataset or a vector from the data space. The objective for summarization is minimize or maximize the cost function $f(A, X)$ for A. This cost function captures the desired properties of the summary such as representativeness and diversity.

The prototypes $A$ can come from dataset, in this case the optimization objective is to search for $A \in 2^{| X |}$, whereas if it come from data space, it is not constrained to be so. The first scenario is achieved by discrete optimization of some cost function over exponential number of possibility. If the cost function is submodular monotone, the greedy search algorithm works with bounded approximation guarantees \cite{nemhauser1978analysis}.

\subsection{Maximum Mean Discrepancy(MMD) for Summarization}
\subsubsection{Maximum Mean Discrepancy (MMD)}

MMD is a metric that measures the distance between two distributions \cite{gretton2012kernel}, by computing differences in mean feature embeddings in some feature space. 

Let $x \sim X, a \sim A$ be the observations from two distributions $X, A$ defined on $\mathcal{X}$, Let $\phi: \mathcal{X} \to \mathcal{H}$ be the feature map defined by reproducing kernel Hilbert space (RKHS $\mathcal{H}$) and $\mathcal{F}$ be the class of smooth functions $f \in \mathcal{F} : \mathcal{H} \to \mathbb{R}$. MMD is defined by the class $\mathcal{F}$ of smooth functions, and it is the difference in expected function values between two samples when this is large. The class $\mathcal{F}$ should be such that the MMD vanishes if and only if $X = A$.
\begin{equation}
    MMD(\mathcal{F}, X, A) = \sup_{f \in \mathcal{F}} ( \mathbb{E}_{x} [f(\phi(x))] - \mathbb{E}_{a} [f(\phi(a))] ) \label{eqn::mmd_1}
\end{equation}

Simplifying \eqref{eqn::mmd_1}, MMD is the difference in mean feature embeddings in $\mathcal{H}$. The use of feature map $\phi$ ensures the higher order moments are also matched, not just the mean.
\begin{align}
 MMD(\mathcal{F}, X, A) &= \| \mathbb{E}_{x} \phi(x) - \mathbb{E}_{y} \phi(a) \|_{\mathcal{H}}  \label{eqn::mmd_2}
\end{align}

This involves evaluating the arbitrarily large dimensional features explicitly. Instead, calculating $MMD^2(\mathcal{F}, X, A)$ and using kernel trick will only need to compute the pairwise kernel defined by $\mathcal{H}$, e.g. rbf kernel.
\begin{align}
    MMD^2(\mathcal{F}, X, A) =&  \mathbb{E}_{x,x'} [k(x,x')] - 2 \times \mathbb{E}_{x,a} [k(x,a)] + \nonumber \\ 
    & \mathbb{E}_{a,a'} [k(a,a') ]  \label{eqn::mmd2}
\end{align}
% Empirically, the biased estimate of MMD can be calculated as:
% \begin{align}
%     MMD^2(\mathcal{F}, X, Y) =& \frac{1}{ | X  | ^2}\sum_{i, j} k(x_i, x_j) - \frac{2}{ | X  |  | Y  |}\sum_{i, j} k(x_i, y_j) + \nonumber \\
%     & \frac{1}{ | Y  | ^2}\sum{i, j} k(y_i, y_j) \label{eqn::mmd2_biased}
% \end{align}
\paragraph{The witness function} of MMD is the function attaining suprenum in \eqref{eqn::mmd_1}.
\begin{align}
    f_{mmd}(z) = \mathbb{E}_x [k(x,z)] - \mathbb{E}_y [k(y,z)] \label{eqn::mmd_witness}
\end{align}

\subsubsection{MMD-Critic}

Kim et al introduced MMD-critic \cite{kim2016examples}, which use MMD to find the prototypes $X_S$ (with indices in dataset as $S$) and then criticisms $X_C$ (with indices in dataset as $C$), both are the samples from dataset. In their method, Prototypes are selected by greedily maximizing $-MMD^2(\mathcal{F}, X_S, X)$ between dataset $X$ (with indices as $V$) and prototypes $X_S$. After that, Criticisms $X_C$ are selected, the data points that are not well characterized by prototypes. This objective is defined by the peaks in witness function of MMD \eqref{eqn::mmd_witness} and log-determinant of the kernel submatrix of criticisms, which acts as diversity regularizer $ {\sum_{c \in C} {\left | {\frac{1}{n}\sum_{i \in V}k(x_i, x_c) - \frac{1}{m}\sum_{j \in S}k(x_j, x_c)  }  \right | }} + \log \mathrm{det}{\ K_{C,C}}$ . Both objectives are submodular-monotone \footnote{log-det is monotone if every eigenvalue of $K_{C, C}$ is greater than or equal to 1} and hence greedy algorithm can be used to get approximate solutions with some bounded guarantees \cite{nemhauser1978analysis}.


\subsection{Time Aware Summarization}
We formulate the time aware summarization as summarization of labeled data, where different time ranges are treated as labels. In this scenario, we are trying to learn a set of prototypes for each time range or label such that the summaries captures what's different compared to other time ranges effectively.

Let us consider that our dataset is labelled and $X = (X_1, X_2  \ldots X_K)$ be the data from K classes. Now the goal is to learn prototypes (let's ignore criticisms and consider summaries contains prototypes only) $A = (A_1, A_2 \ldots A_K)$ such that the prototypes are different from each other.

\subsection{MMD for Time Aware Summarization}
In presence of labeled data, where goal to learn distinctive prototypes for different labels, MMD can be leveraged as
\begin{equation}
	 \argmax_{A_1, A_2 \ldots A_K} \sum_{k} \bigg( -MMD^2(\mathcal{F}, A_k, X_k) + \lambda MMD^2(\mathcal{F}, A_k, X_{\sim k})  \bigg)\label{eqn::mmd_labels}
\end{equation}  
The first term is learning prototypes for each labels, whereas the second term is trying to make prototypes distinctive my making them different than data points from other time ranges. 

\subsubsection{Greedy Optimization}
The objective is no longer submodular, but, we can still optimize using greedy algorithm as outlined in \ref{algo::greedy_max_mmd_labels}, without approximation guarantees. Here the optimization function $\sum_k F(S_k; V, X) $ because the prototypes $A_k$ come from the dataset and we denote them with $X_{S_k}$, and we optimize for $S = (S_1, S_2, \ldots S_K) $, where $S_k$ denotes the indices from datasets for prototypes of class $k$. Let $V_k$ denote the indices of data points from class $k$ and $V = (V_1, V_2 \ldots V_k)$

\begin{algorithm}
    \caption{Greedy algorithm to maximize $\sum_k F(S_k; V, X) = \sum_k ( -MMD^2(\mathcal{F}, X_{S_k}, X_k) + \lambda MMD^2(\mathcal{F}, X_{S_k}, X_{\sim k})) $} \label{algo::greedy_max_mmd_labels}
    \begin{algorithmic}[1]
        \Require{$X: Dataset, V = (V_1, V_2 \ldots V_k)$, m: number of prototypes/crictisms}
        \Procedure{maximize}{$X, V, m$}
        \State $\forall_{k \in 1 \ldots K} S_k\gets \{ \}$
        \While{$ \forall_{k \in 1 \ldots K} | S_k  | \leq m $}
            \State $s_k^{*} \gets \argmax_{s:\forall s \in V_k} F(S_k \cup {s}; V, X) - F(S_k; V, X)$
            \State $S_k \gets S_k \cup {s^{*}}$
            \State $V_k \gets V_k - {s^{*}}$
        \EndWhile
        \State $S \gets (S_1, S_2 \ldots S_K)$
        \State \textbf{return} $S$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\subsubsection{Gradient Based optimization}
Alternatively, the objective can be optimized using gradient based methods. The equation and gradient for $MMD^2(\mathcal{F}, A, X)$ is defined as:
\begin{align}
    MMD^2(\mathcal{F}, A, X) =& \frac{-2}{m \times n}\sum_{i=1}^n\sum_{j=1}^m k(x_i, a_j) + \frac{1}{m^2}\sum_{i, j = 1}^m k(a_i, a_j) \label{eqn::mmd_emperical}\\
\nabla_{a_l} MMD^2(\mathcal{F}, A, X) =& \frac{4\gamma}{m} \bigg(\frac{-1}{n} \sum_{i = 1}^{n} {k(x_i, a_l)(x_i - a_l) } + \nonumber\\ &\ \frac{1}{m^2} \sum_{i = 1}^{m} {k(a_i, a_l)(a_i - a_l) }  \bigg) \label{eqn::mmd_grad}
\end{align}

Compared to \eqref{eqn::mmd2}, \eqref{eqn::mmd_emperical} doesn't has first term because it is constant and doesn't matter in the optimization.
The other variant of making distinctive prototypes is to make them different from prototypes of other classes.
\begin{equation}
	 \argmax_{A_1, A_2 \ldots A_K} \sum_{k} \bigg( -MMD^2(\mathcal{F}, A_k, X_k) + \lambda MMD^2(\mathcal{F}, A_k, A_{\sim k})  \bigg)\label{eqn::mmd_labels2}
\end{equation}
The gradient of second term is different than \eqref{eqn::mmd_grad}. Let $I(k)$ be the list of indices of $A$ corresponding to class $k$. And, first term of $MMD^2$ can no longer be ignored like in \eqref{eqn::mmd_emperical}
\begin{align}
\begin{split}
\nabla_{a_l} MMD^2(\mathcal{F}, A_k, A_{\sim k}) =\\
        \begin{cases}
            \displaystyle 4\gamma \bigg(\frac{1}{m_k^2}\sum_{i \in I(k)}(a_i - a_l)k(a_i, a_l) -\\ \displaystyle \frac{1}{m_k m_{\sim k}}\sum_{i \notin I(k)}(a_i - a_l)k(a_i, a_l) \bigg), & \text{if $l \in I(k)$}  \\
            \displaystyle 4\gamma \bigg(\frac{1}{m_{\sim k}^2}\sum_{i \notin I(k)}(a_i - a_l)k(a_i, a_l) -\\ \displaystyle \frac{1}{m_k m_{\sim k}}\sum_{i \in I(k)}(a_i - a_l)k(a_i, a_l) \bigg), & \text{if $l \notin I(k)$}
        \end{cases}
    \end{split} \label{eqn::mmd_grad_protos}
\end{align}
where $l \in 1 \ldots m$
